The Vault: A Comprehensive Multilingual Dataset for Advancing Code Understanding and Generation

We present The Vault, a dataset of high-quality code-text pairs in multiple programming languages for training large language models to understand and generate code. We present methods for thoroughly extracting samples that use both rule-based and deep learning-based methods to ensure that they contain high-quality pairs of code and text, resulting in a dataset of 43 million high-quality code-text pairs. Our extensive evaluations on common coding tasks including code generation, code search and code summarization show that when fine-tuning Code Large Language Models on The Vault, such models outperform the same models trained on other datasets such as CodeSearchNet. We also provide detailed analyses of our datasets to assess the effects of various programming languages and docstrings on the performance of such models.

==> tmp.tex <==

\begin{document}

\begin{table}[t!]
\scriptsize
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{l|r|r|rr}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Repo}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\#Language\end{tabular}}} & \multicolumn{2}{c}{\#Function} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & w/ docstring & w/o docstring \\ \hline \hline
PyMT5 \citep{DBLP:conf/emnlp/ClementDTSS20} & - & 1 & $\approx$ 7,700,000 & - \\
CoDesc \citep{HasanMIMHHAIS21} & - & 1 & 4,211,516 & - \\
CodeSearchNet \citep{husain2019codesearchnet} & - & 6 & 2,326,976 & 4,125,470 \\
CodeSearchNet (CodeXGLUE \citep{DBLP:conf/nips/LuGRHSBCDJTLZSZ21}) & - & 6 & 1,005,474 & - \\
Deepcom \citep{HuLXLJ20} & 9,714 & 1 & 424,028 & - \\
CONCODE \citep{iyer-etal-2018-mapping} & 33,000 & 1 & 2,184,310 & - \\
Funcom \citep{DBLP:conf/icse/LeClairJM19} & 28,000 & 1 & 2,149,121 & - \\
\cite{9054866} & - & 1 & 164,937 & - \\
CodeT5 \citep{DBLP:conf/emnlp/0034WJH21} & - & 8 & 3,158,313 & 5,189,321 \\ \hline
\textit{\textbf{The Vault}} & \textit{\textbf{2,369,844}} & \textit{\textbf{10}} & \textit{\textbf{41,206,602}} & \textit{\textbf{205,151,985}} \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of the Vault to other code-text datasets. The symbol "-" means the information is not given.}
\label{table_comparation_function}
\end{table}

\end{document}
